Fairness Testing through Extreme Value Theory

Data-driven software is increasingly being used as a critical component of automated decision-support systems. Since this class of software learns its logic from historical data, it can encode or amplify discriminatory practices. Previous research on algorithmic fairness has focused on improving average-case fairness. On the other hand, fairness at the extreme ends of the spectrum, which often signifies lasting and impactful shifts in societal attitudes, has received significantly less emphasis. Leveraging the statistics of extreme value theory (EVT), we propose a novel fairness criterion called extreme counterfactual discrimination (ECD). This criterion estimates the worst-case amounts of disadvantage in outcomes for individuals solely based on their memberships in a protected group. Utilizing tools from search-based software engineering and generative AI, we present a randomized algorithm that samples a statistically significant set of points from the tail of ML outcome distributions even if the input dataset lacks a sufficient number of relevant samples. We conducted several experiments on four ML models (deep neural networks, logistic regression, and random forests) over 10 socially relevant tasks from the literature on algorithmic fairness. First, we evaluate the generative AI methods and find that they generate sufficient samples to infer valid EVT distribution in 95% of cases. Remarkably, we found that the prevalent bias mitigators reduce the average-case discrimination but increase the worst-case discrimination significantly in 5% of cases. We also observed that even the tail-aware mitigation algorithm -- MiniMax-Fairness -- increased the worst-case discrimination in 30% of cases. We propose a novel ECD-based mitigator that improves fairness in the tail in 90% of cases with no degradation of the average-case discrimination.

==> Sections/CV_Plots.tex <==
\begin{figure*}
    \centering
    \includegraphics[width = 0.24\textwidth]{Figures/CV_plots/census_sex_female_cvplot.png} 
    \includegraphics[width = 0.24\textwidth]{Figures/CV_plots/census_sex_male_cvplot.png}
    \includegraphics[width = 0.24\textwidth]{Figures/CV_plots/compas_race_non-caucasian_cvplot.png} 
    \includegraphics[width = 0.24\textwidth]{Figures/CV_plots/compas_race_caucasian_cvplot.png}
    \caption{\textit{The Exponentially Test with CV during Search}: (Left) Census with Sex=Female; (Mid-Left) Census with Sex=Male; (Mid-Right) Compas with Race=Non-Caucasian; (Right) Compas with Race=Caucasian.}
    \label{fig:CV_test}
    \vspace{-1.0em}
\end{figure*}

==> Sections/RQ-1-Table-append.tex <==
\begin{table*}[tbp!]
    \caption{Characteristics of Extreme Value Distributions. 
      Legend: (\textit{Dataset})
      \textbf{P}: Protected Attribute,
      \textbf{\#N}: Number of test cases,
      \textbf{ACD}: Average counterfactual discrimination.
      (\textit{EVT Characteristics})
      ($\mu, \sigma, \xi$, type) for parameters of distributions,
      \textbf{$\tau$}: threshold.
      (\textit{Feasibility}) EVT-based extrapolation based on Q-Q Plot and its upper-bounds (B) on the number of interactions. ($\epsilon$ denotes positive values less than 0.01).
    }
    \label{tab:EVT-validity-guarantee}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{ | l | l  l  r l | l  l  l  l  l | l  l  | }
      \hline
      & \multicolumn{4}{c|}{Dataset}  & \multicolumn{5}{c|}{EVT Characteristics} & \multicolumn{2}{c|}{Feasibility}
      \\
    Algorithm & Name  & P & \#N & ACD & $\mu$ & $\sigma$ & $\xi$ & $\tau$ & Type & Q-Q Plot & B  \\ \hline
 
 \multirow{14}{*}{Gradient boosting} & \multirow{2}{*}{Census} & R=White &  25,658&-0.01&0.1(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-0.13(+/- $\epsilon$)&0.09 &  III-Finite & Linear & $\infty$ \\
    &  & R=Black & 3,076&0.01&0.06(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-0.11(+/- $\epsilon$)&0.05 & III-Finite & Linear & $\infty$\\ \cline{2-12}
     & \multirow{2}{*}{Census} & S=Male &  10,249&0.0&0.08(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-0.03(+/- $\epsilon$)&0.07 & I-Log &  & \\
    &  & S=Female & 20,100&-0.03&0.02(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-0.04(+/- $\epsilon$)&0.01 & I-Log &  & \\ \cline{2-12}
     & \multirow{2}{*}{Credit} & S=Female & 310&-0.01&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-1.09(+/- $\epsilon$)&0.0&  III-Finite & Linear & $\infty$ \\
    &  & S=Male & 688&0.02&0.11(+/- $\0.01$)&0.03(+/- $\0.01$)&-0.37(+/- $\0.01$)&0.06 & III-Finite & Linear & $\infty$ \\ \cline{2-12}
     & \multirow{2}{*}{Bank} & A=Young &  9,9450&0.0&0.02(+/- $\epsilon$)&0.02(+/- $\epsilon$)&0.84(+/- $\epsilon$)&0.01 &  II-Infinite & Heavy-Tail & 0 \\
    &  & A=Old & 1,487&0.0&0.03(+/- $\epsilon$)&0.01(+/- $\epsilon$)&0.02(+/- $\epsilon$)&0.02 & I-Log &  &  \\ \cline{2-12}
     & \multirow{2}{*}{Compas} & S=Male & 3,527&0.01&0.06(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-0.06(+/- $\epsilon$)&0.05 &  III-Finite & Linear & $\infty$ \\
    &  & S=Female & 1,407&0.0&0.04(+/- $\epsilon$)&0.04(+/- $\epsilon$)&0.32(+/- $\epsilon$)&0.02 & II-Infinite & Linear & $\infty$ \\ \cline{2-12}    
     & \multirow{2}{*}{Compas} & R=Caucasian & 2,969&0.02&0.07(+/- $\epsilon$)&0.02(+/- $\epsilon$)&0.39(+/- $\epsilon$)&0.06 & II-Infinite & Heavy-Tail & 0 \\     
      &  &  R=Non-Caucasian & 1,941&-0.01&0.01(+/- $\epsilon$)&0.01(+/- $\epsilon$)&0.0(+/- $\epsilon$)&0.0 &  I-Log &  &  \\ \cline{2-12}        
     & \multirow{2}{*}{Compas} & A=Young & 3,154&-0.02&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-1.0(+/- $\epsilon$)&0.0&   III-Finite & Linear & $\infty$ \\
    &  & A=Old & 839&0.01&0.1(+/- $0.02$)&0.05(+/- $0.02$)&0.02(+/- $0.02$)&0.04 & I-Log &  &  \\  \cline{2-12}
    & \multirow{2}{*}{Default} & S=Male &  11,391&-0.01&0.08(+/- $0.01$)&0.04(+/- $0.01$)&0.04(+/- $0.01$)&0.04 & I-Log &  &  \\     
      &  &  S=Female & 17,211&0.01&0.11(+/- $0.01$)&0.04(+/- $0.01$)&0.05(+/- $0.01$)&0.07 &  I-Log &  & \\ \cline{2-12}
    & \multirow{2}{*}{Heart} & S=Male & 680&0.02&0.08(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-0.63(+/- $\epsilon$)&0.06 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 201&-0.01&0.02(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-0.06(+/- $\epsilon$)&0.01 & III-Finite & Linear & $\infty$ \\ \cline{2-12}
      & \multirow{2}{*}{Meps15} & S=Male &   8,250&-0.03&0.07(+/- $\epsilon$)&0.02(+/- $\epsilon$)&0.11(+/- $\epsilon$)&0.05 & II-Infinite &  Heavy-Tail & 0  \\     
      &  &  S=Female & 7,580&0.02&0.2(+/- $0.04$)&0.05(+/- $0.04$)&-0.4(+/- $0.04$)&0.15 &  III-Finite & Linear & $\infty$  \\ \cline{2-12}
      & \multirow{2}{*}{Meps16} & S=Male & 8,298&-0.05&0.02(+/- $\epsilon$)&0.01(+/- $\epsilon$)&0.1(+/- $\epsilon$)&0.01 & II-Infinite &  Heavy-Tail & 0  \\     
      &  &  S=Female & 7,377&0.04&0.21(+/- $\epsilon$)&0.04(+/- $\epsilon$)&0.34(+/- $\epsilon$)&0.18 &  II-Infinite &  Heavy-Tail & 0 \\ \cline{2-12}
      & \multirow{2}{*}{Students} & S=Male & 590&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-479.57(+/- $\epsilon$)&0.0 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female &  1,321&0.01&0.04(+/- $\epsilon$)&0.01(+/- $\epsilon$)&0.14(+/- $\epsilon$)&0.03 &  II-Infinite &  Heavy-Tail & 0  \\ \cline{2-12}\hline 

     \multirow{14}{*}{Bagging} & \multirow{2}{*}{Census} & R=White & 25,658&-0.01&0.64(+/- $0.05$)&0.09(+/- $0.05$)&-0.42(+/- $0.05$)&0.5 &  III-Finite & Linear & $\infty$ \\
    &  & R=Black & 3,076&0.01&0.54(+/- $0.03$)&0.13(+/- $0.03$)&-0.16(+/- $0.03$)&0.4 & III-Finite & Linear & $\infty$\\ \cline{2-12}
     & \multirow{2}{*}{Census} & S=Male & 10,249&0.02&0.71(+/- $0.04$)&0.08(+/- $0.04$)&-0.47(+/- $0.04$)&0.6 & III-Finite & Linear & $\infty$\\
    &  & S=Female & 20,100&0.0&0.57(+/- $\epsilon$)&0.07(+/- $\epsilon$)&-1.14(+/- $\epsilon$)&0.4 & III-Finite & Linear & $\infty$\\ \cline{2-12}
     & \multirow{2}{*}{Credit} & S=Female & 829&0.0&0.01(+/- $\epsilon$)&0.03(+/- $\epsilon$)&-2.68(+/- $\epsilon$)&-0.1&  III-Finite & Linear & $\infty$ \\
    &  & S=Male & 688&0.01&0.11(+/- $0.02$)&0.04(+/- $\0.02$)&-0.5(+/- $0.02$)&0.0 & III-Finite & Linear & $\infty$ \\ \cline{2-12}
     & \multirow{2}{*}{Bank} & A=Young &  9,458&0.0&0.3(+/- $\epsilon$)&0.07(+/- $\epsilon$)&-1.0(+/- $\epsilon$)&0.2 &  III-Finite & Linear & $\infty$\\
    &  & A=Old & 1,487&0.0&0.2(+/- $0.04$)&0.09(+/- $0.04$)&-0.22(+/- $\0.04$)&0.1 & III-Finite & Linear & $\infty$ \\ \cline{2-12}
     & \multirow{2}{*}{Compas} & S=Male & 3,527&-0.01&0.58(+/- $0.03$)&0.13(+/- $0.03$)&0.0(+/- $0.03$)&0.44  &  I-Log &  & \\
    &  & S=Female & 906&-0.01&0.39(+/- $0.17$)&0.22(+/- $0.17$)&-0.81(+/- $0.17$)&0.1  & III-Finite & Linear & $\infty$ \\ \cline{2-12}    
     & \multirow{2}{*}{Compas} & R=Caucasian & 2,969&0.01&0.67(+/- $0.05$)&0.13(+/- $0.05$)&-0.33(+/- $0.05$)&0.5  & III-Finite & Linear & $\infty$ \\     
      &  &  R=Non-Caucasian & 1,464&-0.02&0.38(+/- $0.04$)&0.13(+/- $0.04$)&-0.32(+/- $0.04$)&0.2  &  III-Finite & III-Finite & Linear & $\infty$ \\ \cline{2-12}        
     & \multirow{2}{*}{Compas} & A=Young & 2,559&-0.03&0.41(+/- $0.04$)&0.1(+/- $0.04$)&-0.38(+/- $0.04$)&0.3 &   III-Finite & Linear & $\infty$ \\
    &  & A=Old & 839&0.01&0.42(+/- $0.06$)&0.17(+/- $0.06$)&-0.36(+/- $0.06$)&0.2  & III-Finite & Linear & $\infty$ \\  \cline{2-12}
    & \multirow{2}{*}{Default} & S=Male & 11,391&-0.01&0.76(+/- $0.02$)&0.1(+/- $0.02$)&-0.87(+/- $0.02$)&0.6 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 17,211&0.02&0.73(+/- $0.03$)&0.08(+/- $0.03$)&-0.4(+/- $0.03$)&0.6 &  III-Finite & Linear & $\infty$  \\ \cline{2-12}
    & \multirow{2}{*}{Heart} & S=Male & 694&0.08&0.3(+/- $\epsilon$)&0.02(+/- $\epsilon$)&-1.24(+/- $\epsilon$)&0.2 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 774&-0.02&0.01(+/- $\epsilon$)&0.03(+/- $\epsilon$)&-0.48(+/- $\epsilon$)&-0.1 &  III-Finite & Linear & $\infty$ \\ \cline{2-12}
      & \multirow{2}{*}{Meps15} & S=Male &  8,250&-0.01&0.48(+/- $0.03$)&0.11(+/- $0.03$)&-0.12(+/- $0.03$)&0.37 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 7,580&0.02&0.47(+/- $\epsilon$)&0.07(+/- $\epsilon$)&-1.0(+/- $\epsilon$)&0.37 &  III-Finite & Linear & $\infty$ \\ \cline{2-12}
      & \multirow{2}{*}{Meps16} & S=Male & 8,298&-0.03&0.56(+/- $0.13$)&0.12(+/- $0.13$)&-0.67(+/- $0.13$)&0.4 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 7,377&0.04&0.61(+/- $0.02$)&0.07(+/- $0.02$)&-0.29(+/- $0.02$)&0.5 &  III-Finite & Linear & $\infty$ \\ \cline{2-12}
      & \multirow{2}{*}{Students} & S=Male & 0&0&0.00&0&0&0.0 & -- & &  \\     
      &  &  S=Female &  0&0&0.00&0&0&0.0 &  -- &  & \\ \cline{2-12}\hline 
      

    \multirow{14}{*}{GNB} & \multirow{2}{*}{Census} & R=White &   0&0&0.00&0&0&0.0 &  - & - & - \\
    &  & R=Black &  0&0&0.00&0&0&0.0 & I-Log & Skewed-Right & - \\ \cline{2-12}
     & \multirow{2}{*}{Census} & S=Male &  10,249&0.02&0.46(+/- $\epsilon$)&0.04(+/- $\epsilon$)&-1.0(+/- $\epsilon$)&0.4 & II-Infinite & Heavy-Tail & 0 \\
    &  & S=Female &  20100&-0.11&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&0.0 & I-Log & Skewed-Right & 2,000 \\ \cline{2-12}
     & \multirow{2}{*}{Credit} & S=Female & 310&-0.04&-0.01(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-1.11(+/- $\epsilon$)&-0.01&  III-Finite & Linear & $\infty$ \\
    &  & S=Male & 688&0.04&0.07(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-1.12(+/- $\epsilon$)&0.07 & III-Finite & Linear & $\infty$ \\ \cline{2-12}
     & \multirow{2}{*}{Bank} & A=Young &  0&0&0.00&0&0&0.0 &  II-Infinite & Heavy-Tail & 0 \\
    &  & A=Old & 0&0&0.00&0&0&0.0 & I-Log & Skewed-Right & 1,000 \\ \cline{2-12}
     & \multirow{2}{*}{Compas} & S=Male & 3,527&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-14.74(+/- $\epsilon$)&0.0 &  III-Finite & Linear & $\infty$ \\
    &  & S=Female & 906&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-0.25(+/- $\epsilon$)&0.0 & III-Finite & Linear & $\infty$ \\ \cline{2-12}    
     & \multirow{2}{*}{Compas} & R=Caucasian & 15,554&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-2.5(+/- $\epsilon$)&0.0& III-Finite & Linear & $\infty$ \\     
      &  &  R=Non-Caucasian & 1,464&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-0.22(+/- $\epsilon$)&0.0 &  I-Log & Skewed-Right & 2,000 \\ \cline{2-12}        
     & \multirow{2}{*}{Compas} & A=Young & 3,162&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-69.15(+/- $\epsilon$)&0.0&   III-Finite & Linear & $\infty$ \\
    &  & A=Old & 839&0.0&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-0.2(+/- $\epsilon$)&0.0 & III-Finite & Linear & $\infty$ \\  \cline{2-12}
    & \multirow{2}{*}{Default} & S=Male & 0&0&0.00&0&0&0.0 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 0&0&0.00&0&0&0.0 &  I-Log & Skewed-Right & 2,000 \\ \cline{2-12}
    & \multirow{2}{*}{Heart} & S=Male & 674&0.06&0.31(+/- $\epsilon$)&0.02(+/- $\epsilon$)&-1.82(+/- $\epsilon$)&0.26 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 201&-0.06&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&-3.56(+/- $\epsilon$)&0.0 &  I-Log & Skewed-Right & 2,000 \\ \cline{2-12}
      & \multirow{2}{*}{Meps15} & S=Male &    0&0&0.00&0&0&0.0 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 0&0&0.00&0&0&0.0 &  I-Log & Skewed-Right & 2,000 \\ \cline{2-12}
      & \multirow{2}{*}{Meps16} & S=Male & 6022&0.0&0.22(+/- $\epsilon$)&0.01(+/- $\epsilon$)&-1.67(+/- $\epsilon$)&0.2 & III-Finite & Linear & $\infty$ \\     
      &  &  S=Female & 6022&-0.01&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&0.0(+/- $\epsilon$)&0.0 &  I-Log & Skewed-Right & 2,000 \\ \cline{2-12}
      & \multirow{2}{*}{Students} & S=Male & 0&0&0.00&0&0&0.0& III-Finite & Linear & $\infty$ \\     
      &  &  S=Female &  0&0&0.00&0&0&0.0 &  I-Log & Skewed-Right & 2,000 \\ \cline{2-12}\hline 
   
    \end{tabular}
 }
 % \vspace{-0.5em}
\end{table*}

==> Sections/RQ-2-Table-append.tex <==
\begin{table*}[tbp!]
    \caption{Characteristics of Extreme Value Distributions. 
      Legend: (\textit{Dataset})
      \textbf{P}: Protected Attribute,
      \textbf{\#N}: Number of test cases,
      \textbf{ACD}: Average counterfactual discrimination.
      (\textit{EVT Characteristics})
      ($\mu, \sigma, \xi$, type) for parameters of distributions,
      \textbf{$\tau$}: threshold.
      (\textit{Feasibility}) EVT-based extrapolation based on Q-Q Plot and its upper-bounds (B) on the number of interactions. ($\epsilon$ denotes positive values less than 0.01).
    }
    
    \label{tab:EVT-validity-guarantee}
    \resizebox{0.7\textwidth}{!}{ 
      \begin{tabular}{ | l | l  l  r l | l  l  l  l  l | l  l  | }
      \hline
      & \multicolumn{4}{c|}{Dataset}  & \multicolumn{5}{c|}{EVT Characteristics} & \multicolumn{2}{c|}{Feasibility}
      \\
    Algorithm & Name  & P & \#N & ACD & $\mu$ & $\sigma$ & $\xi$ & $\tau$ & Type & Q-Q Plot & B  \\ \hline
   

    \multirow{7}{*}{Gradient Boosting} & \multirow{2}{*}{Census} & Race & 0.86&0.03&0.04&0.02&-0.04&-0.02&-0.04&-0.04&-0.05&-0.06 \\
    & & Sex & 0.86&0.12&0.08&-0.03&-0.07&-0.07&-0.08&-0.08&-0.08&-0.07 \\ \cline{2-13}
    & Credit & Sex &  0.79&0.21&0.12&0.03&0.11&0.2&0.21&0.22&0.23&0.23\\ \cline{2-13}
    & Bank & Age & 0.91&0.19&0.09&0.0&0.01&0.03&0.03&0.04&0.05&0.04 \\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex & 0.95&0.0&0.03&-0.01&-0.02&0.02&0.03&0.06&0.11&0.14 \\  
    &  &  Race &  0.95&0.0&0.03&-0.03&-0.07&-0.08&-0.09&-0.11&-0.14&-0.18 \\
    & &  Age &0.95&0.0&0.0&0.02&0.09&0.19&0.23&0.26&0.31&0.35 \\ \cline{2-13}
    & Default & Sex &  0.82&0.02&0.02&0.03&0.03&-0.01&-0.01&-0.02&-0.02&-0.02 \\ \cline{2-13}
    & Heart & Sex &  0.84&0.47&0.27&-0.03&-0.05&-0.04&-0.03&-0.02&-0.01&-0.01 \\ \cline{2-13}
    & Meps15 & Sex & 0.87&0.07&0.05&0.05&0.13&0.06&0.1&0.12&0.14&0.14 \\ \cline{2-13}
    & Meps16 & Sex & 0.86&0.06&0.05&0.09&0.19&0.18&0.18&0.19&0.22&0.25\\ \cline{2-13}
    & Students & Sex & 0.9&0.01&0.0&0.01&0.04&0.07&0.08&0.09&0.11&0.12 \\ \cline{2-13}\hline

    \multirow{7}{*}{Bagging} & \multirow{2}{*}{Census} & Race & 0.83&0.03&0.01&0.02&-0.05&0.29&0.22&0.18&0.17&0.16 \\
    & & Sex &0.83&0.01&0.01&-0.02&-0.2&-0.28&-0.18&-0.16&-0.17&-0.19 \\ \cline{2-13}
    & Credit & Sex & 0.77&0.07&0.01&0.01&0.01&0.17&0.18&0.19&0.2&0.2 \\ \cline{2-13}
    & Bank & Age & 0.9&0.11&0.06&0.0&-0.1&0.11&0.05&0.04&0.05&0.07 \\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex &0.92&0.01&0.03&0.0&-0.29&0.07&-0.01&-0.08&-0.19&-0.28 \\  
    &  &  Race & 0.92&0.01&0.01&-0.04&-0.23&-0.18&-0.2&-0.21&-0.22&-0.22 \\
    & &  Age &0.92&0.0&0.01&0.03&-0.02&0.24&0.26&0.26&0.28&0.28 \\ \cline{2-13}
    & Default & Sex & 0.79&0.02&0.02&0.03&-0.02&-0.1&-0.1&-0.08&-0.04&-0.02 \\ \cline{2-13}
    & Heart & Sex &  0.84&0.2&0.14&-0.1&-0.3&-0.31&-0.31&-0.3&-0.3&-0.3 \\ \cline{2-13}
    & Meps15 & Sex & 0.84&0.03&0.01&0.03&-0.01&0.06&0.01&-0.04&-0.13&-0.17 \\ \cline{2-13}
    & Meps16 & Sex & 0.85&0.03&0.02&0.07&0.07&0.11&0.06&0.04&0.04&0.05 \\ \cline{2-13}
    & Students & Sex &  0.91&0.01&0.01&0.0&0&0.83&0.5&0.34&0.25&0.22 \\ \cline{2-13}\hline

    \multirow{7}{*}{Gaussian Naive Bayes} & \multirow{2}{*}{Census} & Race &  0.83 & 0.1 & 0.1 & 0.17 &  NV & NV & NV & NV & NV & NV\\
    & & Sex &0.8&0.07&0.06&-0.14&-0.46&-0.47&-0.49&-0.5&-0.51&-0.51\\ \cline{2-13}
    & Credit & Sex & 0.76&0.11&0.06&0.08&0.08&0.07&0.07&0.07&0.07&0.07 \\ \cline{2-13}
    & Bank & Age & 0.8&0.17&0.14&0.0&0.01&0.01&0.01&0.01&0.01&0.01\\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex & 0.95&0.0&0.03&0.0&0&0&0&0&0&0 \\  
    &  &  Race & 0.95&0.0&0.03&0.0&0&0&0&0&0&0 \\
    & &  Age &0.95&0.0&0.0&0.0&0&0&0&0&0&0 \\ \cline{2-13}
    & Default & Sex & 0.62& 0.06 & 0.09 & 0.07 & NV & NV & NV & NV & NV & NV \\ \cline{2-13}
    & Heart & Sex &  0.87 & 0.14 & 0.11& -0.12 & NV & NV & NV & NV & NV & NV \\ \cline{2-13}
    & Meps15 & Sex & 0.67 & 0.11 & 0.07 & -0.03 & NV & NV & NV & NV & NV & NV \\ \cline{2-13}
    & Meps16 & Sex & 0.79  & 0.12 & 0.1 & -0.01 & NV & NV & NV & NV & NV & NV\\ \cline{2-13}
    & Students & Sex &  0.86 & 0.06 & 0.11 & 0.01 & NV & NV & NV & NV & NV & NV\\ \cline{2-13}\hline


    
    \end{tabular}
 }
\end{table*}

==> Sections/RQ-2-Table.tex <==
\setlength{\tabcolsep}{5pt} % Default value: 6pt
\begin{table*}[tbp!]
    \caption{Quantifying and comparing the amounts of bias through EVT.
      Legend:
      \textbf{P}: Protected Attribute,
      \textbf{Acc}: Overall Accuracy,
      \textbf{EOD}: Equal Opportunity Difference,
      \textbf{AOD}: Average Odd Difference,
      \textbf{ACD$^2$} = ACD$_u$-ACD$_p$: Average Counterfactual Discrimination Difference,
      \textbf{ECD$^2$} = $\mu_u-\mu_p$: The Amounts of ECD Tail Discrimination,
      \textbf{RLD}$^2_{n}$: Difference in the Expected Return-Level of $ECD$ in the next $n$ queries,
      \textbf{NV}: Not Valid.           
    }
    \label{tab:tab:EVT-compare-EOD}
    \resizebox{1.0\textwidth}{!}{
      \begin{tabular}{ | l | l  l |  r  r  r  r | l  l  l  l  l  l | }
      \hline
      \multicolumn{3}{|c|}{\textbf{Name}}  &  \multicolumn{4}{c|}{\textbf{Average Cases}} & \multicolumn{6}{c|}{\textbf{Tails Cases}}
      \\
    \multicolumn{1}{|c}{Algorithm}  & Dataset  & P & Acc & $|EOD|$ & $|AOD| $& ACD$^2$ & ECD$^2$ & RLD$^2_{500}$ & RLD$^2_{1,000}$ & RLD$^2_{2,000}$ & RLD$^2_{5,000}$ & RLD$^2_{10,000}$  \\ \hline
    \multirow{12}{*}{DNN} & \multirow{2}{*}{Census} & Race & 0.84&0.07&0.05&\cellcolor{gray!10} 0.07&\cellcolor{gray!25} 0.13&0.26&0.29&0.32&0.34&0.36 \\
    & & Sex & 0.84&0.15&0.12&\cellcolor{gray!10} 0.06&\cellcolor{gray!45} 0.21& 0.20& 0.28& 0.34& 0.38& 0.39\\ \cline{2-13}
    & Credit & Sex & 0.77&0.17&0.09&\cellcolor{gray!10} 0.05&\cellcolor{gray!10} 0.09&0.11&0.12&0.12&0.12&0.12 \\ \cline{2-13}
    & Bank & Age & 0.90&0.13&0.06&0.0&NV&NV&NV&NV&NV&NV \\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex & 0.95&0.00&0.03&0.00&0.04&\cellcolor{gray!25}0.10&0.10&0.15&0.16&0.18 \\  
    &  &  Race &  0.94&0.0&0.03& 0.02 & \cellcolor{gray!25}0.10& 0.11& 0.13& 0.14& 0.15& 0.17 \\
    & &  Age & 0.95&0.0&0.0&\cellcolor{gray!10} 0.07&NV&NV&NV&NV&NV&NV \\ \cline{2-13}
    & Default & Sex & 0.81&0.01&0.02&0.03&NV&NV&NV&NV&NV&NV\\ \cline{2-13}
    & Heart & Sex & 0.76&0.07&0.08&-0.01&-0.01&-0.02&-0.02&-0.02&-0.02&-0.03 \\ \cline{2-13}
    & Meps15 & Sex & 0.85&0.06&0.06&\cellcolor{gray!10} 0.05&NV&NV&NV&NV&NV&NV \\ \cline{2-13}
    & Meps16 & Sex & 0.86&0.01&0.02&\cellcolor{gray!10} 0.07&\cellcolor{gray!55} 0.20&0.21&0.21&0.21&0.19&0.18 \\ \cline{2-13}
    & Students & Sex & 0.91&0.04&0.02&0.02&\cellcolor{gray!10} 0.09&0.19&0.20&0.21&0.22&0.23 \\ \cline{2-13}\hline

    \multirow{12}{*}{LR} & \multirow{2}{*}{Census} & Race & 0.81&0.06&0.03&\cellcolor{gray!10} 0.09&\cellcolor{gray!25} 0.11&0.11&0.11&0.11&0.11&0.11 \\
    & & Sex & 0.81&0.14&0.11&\cellcolor{gray!10} 0.06&\cellcolor{gray!10} 0.07& 0.07& 0.07& 0.07 & 0.07 & 0.07\\ \cline{2-13}
    & Credit & Sex & 0.75&0.25&0.16&\cellcolor{gray!25} 0.10&\cellcolor{gray!25} 0.10&0.09&0.08&0.08&0.08&0.08\\ \cline{2-13}
    & Bank & Age & 0.9&0.09&0.04&0.0&0.01&0.01&0.01&0.01&0.01&0.01\\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex & 0.95&0.0&0.03&-0.01&-0.02&-0.02&-0.02&-0.02&-0.02&-0.02 \\  
    &  &  Race &  0.95&0.0&0.03& 0.04 & \cellcolor{gray!10} 0.06 &  0.07 & 0.07 & 0.07 & 0.07 & 0.08 \\
    & &  Age & 0.95&0.00&0.00&0.04&\cellcolor{gray!10} 0.06&0.07&0.08&0.08&0.08&0.08 \\ \cline{2-13}
    & Default & Sex & 0.81&0.05&0.03&0.04&0.03&0.03&0.03&0.03&0.03&0.03 \\ \cline{2-13}
    & Heart & Sex & 0.87&0.07&0.10&-0.02&-0.01&-0.02&-0.02&-0.02&-0.02&-0.02 \\ \cline{2-13}
    & Meps15 & Sex & 0.86&0.08&0.06&\cellcolor{gray!10} 0.06&\cellcolor{gray!10} 0.07&0.07&0.07&0.07&0.07&0.07\\ \cline{2-13}
    & Meps16 & Sex & 0.86&0.11&0.07&\cellcolor{gray!25} 0.10&\cellcolor{gray!25} 0.13&0.12&0.12&0.12&0.12&0.12\\ \cline{2-13}
    & Students & Sex & 0.91&0.00&0.00&0.04&\cellcolor{gray!25} 0.10&0.10&0.10&0.10&0.10&0.10
 \\ \cline{2-13}\hline
    
    \multirow{7}{*}{SVM} & \multirow{2}{*}{Census} & Race & 0.83&0.11&0.06&0.04&0.03&0.16&0.14&0.12&0.11&0.11 \\
    & & Sex & 0.83&0.09&0.06& 0.04 & \cellcolor{gray!45}  0.15& 0.15 & 0.16 & 0.17 & 0.19 & 0.2\\ \cline{2-13}
    & Credit & Sex & 0.71&0.19&0.12&0.01&0.02&0.01&0.01&0.01&0.00&0.00\\ \cline{2-13}
    & Bank & Age & 0.89&0.06&0.04&0.01&-0.07 &0.01&0.01&0.01&0.02&0.02\\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex &  0.94&0.00&0.04&0.00&NV&NV&NV&NV&NV&NV \\  
    &  &  Race & 0.94&0.00&0.04&0.00&NV&NV&NV&NV&NV&NV\\
    & &  Age &0.94&0.00&0.01&0.00&NV&NV&NV&NV&NV&NV\\ \cline{2-13}
    & Default & Sex & 0.81&0.02&0.01&0.00&0.01&0.00&0.01&0.01&0.01&0.01 \\ \cline{2-13}
    & Heart & Sex & 0.75&0.27&0.10&0.00&0.00&-0.01&-0.01&-0.01&-0.01&-0.01\\ \cline{2-13}
    & Meps15 & Sex & 0.86&0.04&0.03&0.02&\cellcolor{gray!10} 0.07&0.08&0.09&0.10&0.10&0.10 \\ \cline{2-13}
    & Meps16 & Sex & 0.86&0.01&0.00&0.03&\cellcolor{gray!25} 0.12&0.13&0.13&0.14&0.14&0.14 \\ \cline{2-13}
    & Students & Sex &  0.92 & 0.01 & 0.03& 0.00& NV& NV&NV&NV&NV&NV\\ \cline{2-13}\hline


    \multirow{7}{*}{RF} & \multirow{2}{*}{Census} & Race & 0.84&0.03&0.02&0.04&0.00&0.21&0.19&0.18&0.15&0.13 \\
    & & Sex & 0.85&0.01&0.01& 0.04& \cellcolor{gray!45}  0.18 &  0.22 &  0.23 &  0.24 & 0.25 & 0.25 \\ \cline{2-13}
    & Credit & Sex & 0.77&0.02&0.00&0.02&0.04&0.05&0.06&0.08&0.11&0.13 \\ \cline{2-13}
    & Bank & Age & 0.91&0.07&0.03&0.01&-0.02&0.05&0.05&0.05&0.06&0.06 \\ \cline{2-13}
    & \multirow{3}{*}{Compas} & Sex & 0.93&0.01&0.03&-0.01&-0.19&0.03&-0.01&-0.07&-0.15&-0.22 \\  
    &  &  Race & 0.93&0.01&0.00& 0.04 & \cellcolor{gray!45} 0.18 & 0.11 &  0.12 &  0.12 &  0.12 &  0.13 \\
    & &  Age & 0.93&0.01&0.01&0.02&-0.07 & 0.09&0.07&0.03&-0.01&-0.04 \\ \cline{2-13}
    & Default & Sex & 0.80&0.03&0.02&0.02&-0.02&-0.04&-0.06&-0.08&-0.11&-0.13\\ \cline{2-13}
    & Heart & Sex &  0.87&0.13&0.12&-0.02&0.00&0.01&0.02&0.02&0.03&0.04 \\ \cline{2-13}
    & Meps15 & Sex & 0.86&0.02&0.02&0.03& -0.13&-0.17&-0.15&-0.11&-0.04&0.01 \\ \cline{2-13}
    & Meps16 & Sex & 0.86&0.03&0.02&\cellcolor{gray!10}0.05&-0.02&-0.03&-0.07&-0.09&-0.11&-0.13 \\ \cline{2-13}
    & Students & Sex & 0.92&0.00&0.04&0.00&0.02&0.02&0.01&0.02&0.01&0.02 \\ \cline{2-13}\hline

    \end{tabular}
 }
\end{table*}

==> Sections/RQ-3-Table_be_Rev.tex <==
\setlength{\tabcolsep}{18.0pt} % Default value: 6pt
\begin{table*}[tbp!]
    \caption{Average based bias mitigation.
    Legend:
      \textbf{P}: Protected Attribute,
      \textbf{Acc loss}:Accuracy loss in mitigation ,
      \textbf{AOD}: Average Odd Difference,
      \textbf{ACD} = ACD$_u$ - ACD$_p$: Average Counterfactual Discrimination Difference,
      \textbf{ECD} = $\mu_u-\mu_p$: The Amounts of ECD Tail Discrimination,
      \textbf{NV}: Not Valid.
    %   Legend:
    % \textbf{P}: Protected Attribute,
    % \textbf{Acc$'$}: Accuracy of mitigated model,
    % \textbf{EOD$'$}: EOD of mitigated model,
    % \textbf{AOD$'$}: AOD of mitigated model,
    % \textbf{ACD$'$}: ACD$^2$ of mitigated model,
    % \textbf{ECD$'$}: ECD$^2$ of mitigated model, 
    % \textbf{RLD}$'_{n}$: RLD for the next $n$ queries for mitigated model.           
    }
    \label{tab:EVT-Bias-Mitigation}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{ | c | l  l |  c  c  c  c  | c  c  c  c  | }
      \hline
      \multicolumn{3}{|c|}{\textbf{Name}}  &  \multicolumn{4}{c|}{\textbf{Exponentiated Gradient~\cite{agarwal2018reductions}}} & \multicolumn{4}{c|}{\textbf{Fair-SMOTE~\cite{10.1145/3468264.3468537}}}
      \\
    \multicolumn{1}{|c}{Algorithm}  & Dataset  & P & Acc loss  & $|AOD|$ & $ACD$  & $ECD$ & Acc loss  & $|AOD| $& $ACD$  & $ECD$ 
    \\ \hline
    \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race & -.02&.02&-.07&-.07&-.05  & .04 & \cellcolor{gray!20}.09 & -.11\\
     & & Sex & -.02&.03&\cellcolor{gray!5}.05& \cellcolor{gray!20}.08&-.05  & .01 & .03 & \cellcolor{gray!100}.28 \\ \cline{2-3}
    & Credit & Sex & -.12&.07&.02&\cellcolor{gray!120}.99&-.12  & .04 & \cellcolor{gray!40}.1 & \cellcolor{gray!60}.15 \\ \cline{2-3}
    DNN & Bank & Age & -.01&.01&.0&-.07&-.03  & .07 & .01 & .04\\ \cline{2-3}
    
     & \multirow{1}{*}{Compas} & Race &  .0&.01&-.03& -.40&-.01 & .02 & .01 & \cellcolor{gray!40}.12\\ \cline{2-3}


    % & \multirow{3}{*}{Compas} & Sex & .0&.01&-.02& -.07&.0  & .02 & -.01 & \cellcolor{gray!45}.12 \\
    % &  &  Race &  .0&.01&-.03& -.40&-.01 & .02 & .01 & \cellcolor{gray!45}.12 \\
    % & &  Age & .0&.01&.04& \cellcolor{gray!45}.45&.0  & .02 & .0 & -.08 \\ \cline{2-3}
     & Default & sex & .01&.01&-.01&-.56&-.02  & .02 & .02 & \cellcolor{gray!5}.05 \\ \cline{2-3}
     & heart & sex & -.09&.03&-.04& -.24&-.06  & .05 & -.01 & .0 \\ \cline{2-3}
     & Meps15 & sex & -.03&.02&.02&\cellcolor{gray!10}.05&-.04  & .04 & .03 & \cellcolor{gray!45}.13\\ \cline{2-3}
     & Meps16 & sex & -.03&.02&.02&\cellcolor{gray!120} .66&-.05  & .03 & .04 & -.03 \\ \cline{2-3}
     & Students & sex & -.05&.01&-.01& .01&.0 & \cellcolor{gray!5}.05 & -.01 & -.03 \\ \cline{2-3}
    \hline
    \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race & -.01&.01&-.05& \cellcolor{gray!120}.54&.03  & .08 & \cellcolor{gray!80}.24 & \cellcolor{gray!80}.2 \\
    & & Sex & -.01&.02&\cellcolor{gray!20}.08& -.26&.02  & .1 & .02 & .01 \\ \cline{2-3}
    & Credit & Sex & -.01&.10&.02& -.01&-0.4 &  .07 & \cellcolor{gray!20}.08 & \cellcolor{gray!40}.1 \\ \cline{2-3}
    LR & Bank & Age & -.09&.07&.01&-.08&.05 &  .32 &\cellcolor{gray!5} .05 & .03 \\ \cline{2-3}
    
     & \multirow{1}{*}{Compas} &  Race &  -.02&.02&-.08& -.44&.01  & .01 & -.03 & -.05\\  \cline{2-3} 
    
    % & \multirow{3}{*}{Compas} & Sex & .0&.02&-.03&-.08&.01 & .02 & -.03 & -.04 \\  
    % &  &  Race &  -.02&.02&-.08& -.44&.01  & .01 & -.03 & -.05 \\
    % & &  Age & .0&.01&-.02 &-.05&.0 & .01 & .02 & .01 \\ \cline{2-3} 
     & Default & sex &.0&.02&.01&\cellcolor{gray!20}.08& .05 & .05 & .01 & .0\\ \cline{2-3}
     & Heart & sex &  -.09&.27&\cellcolor{gray!60}.17&\cellcolor{gray!120}.60&-.05  & .1 & .01 & .01\\ \cline{2-3}
     & Meps15 & sex & -.01&.02&.01&-.16&-.02 & .05 & \cellcolor{gray!5}.05 & \cellcolor{gray!40}.1 \\ \cline{2-3}
     & Meps16 & sex & .0&.02&.02 &\cellcolor{gray!120}.63&-.1&.6&\cellcolor{gray!120}.67&\cellcolor{gray!120}.69 \\ \cline{2-3}
     & Students & sex & -.01  & .02 & \cellcolor{gray!20}.06 & NV & -.07 &NV & NV & NV \\ \cline{2-3}
     \hline
    
    \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race &-.04&.01&.01 &.08&-.04 & .07 &\cellcolor{gray!20} .08 & \cellcolor{gray!20}.08\\
    & & Sex & -.04&.0&.01 &\cellcolor{gray!120}.95&-.04  & .01 & -.03 & -.08\\\cline{2-3}
    & Credit & Sex & -.09&.14&\cellcolor{gray!20}.09 &\cellcolor{gray!110}.32&-.05  & .01 & .03 &\cellcolor{gray!5}.05\\\cline{2-3}
    SVM & Bank & Age & -.03&.05&.01 &.03&-.01  & .02 & .0 & -.04\\\cline{2-3}

    & \multirow{1}{*}{Compas} & Race &  .01&.01&-.02 &-.06&.01  & .01 & .0 & -.04 \\  \cline{2-3}

    % & \multirow{3}{*}{Compas} & Sex &.0&.02&-.04 &-.08&.01  & .02 & .0 & .0 \\  
    % &  &  Race &  .01&.01&-.02 &-.06&.01  & .01 & .0 & -.04 \\
    % & &  Age & .0&.0&-.01 &-.03&.01  & .02 & .0 & -.01 \\\cline{2-3} 
    
     & Default & sex & -.02 &  .0 & .0 & .0 &-.04  & .02 & .0 & -.05 \\\cline{2-3}
     & Heart & sex & -.04&.01&\cellcolor{gray!20}.06&.02&.05  & .06 & .0 & .0\\\cline{2-3}
     & Meps15 & sex & .0&.01&.0 &\cellcolor{gray!120}.42&-.04  & .03 & .04 & \cellcolor{gray!40}.13 \\\cline{2-3}
     & Meps16 & sex & -.02&.0&.01 &\cellcolor{gray!120}.88&-.05  & .04 &\cellcolor{gray!20} .06 & \cellcolor{gray!80}.21 \\\cline{2-3}
     & Students & sex &-.02&.0&\cellcolor{gray!20}.09 &\cellcolor{gray!120}.86&.02  & .04 & -.04 & -.05\\\cline{2-3}\hline

     \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race &-.04&.02&\cellcolor{gray!20}.07&.01&-.02 & .01 & \cellcolor{gray!20}.06 & -.22\\
    & & Sex &-.04&.05&-.04&.0&-.02  & .01 & .01 & \cellcolor{gray!5}.05\\\cline{2-3}
    & Credit & Sex & -.05&.08&\cellcolor{gray!5}.05 &NV & -.07 & .05 & .04 & \cellcolor{gray!40}.12 \\\cline{2-3}
    RF & Bank & Age & -.01&.01&.01 &.01&-.01  & .02 & -.03 & -.12 \\\cline{2-3}

    & \multirow{1}{*}{Compas} &  Race &  -.02&.0&-.03 &.0&.02  & .0 & -.04 & -.28 \\  \cline{2-3}

    % & \multirow{3}{*}{Compas} & Sex & -.01&.02&-.03 &-.03&.0  & .0 & -.02 & .03 \\  
    % &  &  Race &  -.02&.0&-.03 &.0&.02  & .0 & -.04 & -.28 \\
    % & &  Age & -.02&.01&-.02 &.0&.0  & .01 & .05 & -.03\\ \cline{2-3} 
     & Default & sex &-.05&.03&.01&.01&-.07 & .01 & .01 & .0\\\cline{2-3}
     & Heart & sex &  -.06&.07&.03 &.0&.-.05  & .02 & .01 & -.07 \\\cline{2-3}
     & Meps15 & sex & -.04&.06&.04&-.05&-.05 & .01 & .03 & -.26 \\\cline{2-3}
     & Meps16 & sex & -0.4&.0&.0 &.0&-.04  & .01 & .03 & \cellcolor{gray!20}.07\\\cline{2-3}
     & Students & sex & -0.2& .09 & -.01 & NV & .0  & .01 & -.03 & -.09 \\\cline{2-3}\hline
    \end{tabular}
 }
 \vspace{-1.0 em}
\end{table*}



% \setlength{\tabcolsep}{15.0pt} % Default value: 6pt
% \begin{table*}[tbp!]
%     \caption{Average based bias mitigation.
%     Legend:
%       \textbf{P}: Protected Attribute,
%       \textbf{Acc$'$}: Overall Accuracy,
%       \textbf{EOD$'$}: Equal Opportunity Difference,
%       \textbf{AOD$'$}: Average Odd Difference,
%       \textbf{ACD$^2$} = ACD$_u$-ACD$_p$: Average Counterfactual Discrimination Difference,
%       \textbf{ECD$^2$} = $\mu_u-\mu_p$: The Amounts of ECD Tail Discrimination,
%       \textbf{NV}: Not Valid.
%     %   Legend:
%     % \textbf{P}: Protected Attribute,
%     % \textbf{Acc$'$}: Accuracy of mitigated model,
%     % \textbf{EOD$'$}: EOD of mitigated model,
%     % \textbf{AOD$'$}: AOD of mitigated model,
%     % \textbf{ACD$'$}: ACD$^2$ of mitigated model,
%     % \textbf{ECD$'$}: ECD$^2$ of mitigated model, 
%     % \textbf{RLD}$'_{n}$: RLD for the next $n$ queries for mitigated model.           
%     }
%     \label{tab:EVT-Bias-Mitigation}
%     \resizebox{\textwidth}{!}{
%       \begin{tabular}{ | c | l  l |  c  c  c  c  c | c  c  c  c  c  | }
%       \hline
%       \multicolumn{3}{|c|}{\textbf{Name}}  &  \multicolumn{5}{c|}{\textbf{Exponentiated Gradient}} & \multicolumn{5}{c|}{\textbf{Fair-SMOTE~\cite{10.1145/3468264.3468537}}}
%       \\
%     \multicolumn{1}{|c}{Algorithm}  & Dataset  & P & Acc$'$ & $|EOD'|$ & $|AOD'|$ & $ACD^2$  & $ECD^2$ & Acc$'$ & $|EOD'|$ & $|AOD'| $& $ACD^2$  & $ECD^2$
%     \\ \hline
%     \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race & .82&.07&.02&-.07&-.07&.87 & .1 & .04 & .09 & -.11\\
%      & & Sex & .82&.04&.03&\cellcolor{gray!10}.05& \cellcolor{gray!10}.08&.87 & .06 & .01 & .03 & \cellcolor{gray!45}.28 \\\cline{2-3}
%     & Credit & Sex & .66&.09&.07&.02&\cellcolor{gray!65}.99&.78 & .02 & .04 & \cellcolor{gray!10}.1 & \cellcolor{gray!45}.15 \\\cline{2-3}
%     DNN & Bank & Age & .89&.01&.01&.0&-.07&.92 & .05 & .07 & .01 & .04\\\cline{2-3}
%     & \multirow{3}{*}{Compas} & Sex & .95&.0&.01&-.02& -.07&.95 & .01 & .02 & -.01 & \cellcolor{gray!45}.13 \\
%     &  &  Race &  .95&.0&.01&-.03& -.40&.94 & .0 & .02 & .01 & \cellcolor{gray!45}.12 \\
%     & &  Age & .95&.01&.01&.04& \cellcolor{gray!45}.45&.95 & .0 & .02 & .0 & -.08 \\\cline{2-3}
%      & Default & sex & .82&.01&.01&-.01&-.56&.84 & .03 & .02 & .02 & \cellcolor{gray!10}.05 \\\cline{2-3}
%      & heart & sex & .68&.0&.03&-.04& -.24&.92 & .0 & .05 & -.01 & .0 \\\cline{2-3}
%      & Meps15 & sex & .86&.01&.02&.02&\cellcolor{gray!10}.05&.91 & .06 & .04 & .03 & \cellcolor{gray!45}.13\\\cline{2-3}
%      & Meps16 & sex & .85&.06&.02&.02&\cellcolor{gray!55} .66&.91 & .05 & .03 & .04 & -.03 \\\cline{2-3}
%      & Students & sex & .85&.06&.01&-.01& .01&.85 & .02 & .05 & -.01 & -.03 \\\cline{2-3}\hline
    
%     \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race & .80&.0&.01&-.05& \cellcolor{gray!55}.54&.77 & .09 & .08 & \cellcolor{gray!45}.24\cellcolor{gray!45} & \cellcolor{gray!45}.2 \\
%     & & Sex & .80&.02&.02&\cellcolor{gray!10}.08& -.26&.78 & .05 & .1 & .02 & .01 \\\cline{2-3}
%     & Credit & Sex & .70&.15&.10&.02& -.01&.77 & .05 & .07 & \cellcolor{gray!10}.08 & \cellcolor{gray!45}.1 \\\cline{2-3}
%     LR & Bank & Age & .81&.20&.07&.01&-.08&.76 & .06 & .32 & \cellcolor{gray!10}.05 & .03 \\\cline{2-3}
%     & \multirow{3}{*}{Compas} & Sex & .95&.0&.02&-.03&-.08&.94 & .0 & .02 & -.03 & -.04 \\  
%     &  &  Race &  .93&.02&.02&-.08& -.44&.95 & .0 & .01 & -.03 & -.05 \\
%     & &  Age & .95&.0&.01&-.02 &-.05&.95 & .0 & .01 & .02 & .01 \\\cline{2-13} 
%      & Default & sex &.81&.03&.02&.01&\cellcolor{gray!10}.08&.76 & .05 & .05 & .01 & .0\\\cline{2-3}
%      & Heart & sex &  .77&.60&.27&\cellcolor{gray!25}.17&\cellcolor{gray!55}.60&.82 & .01 & .1 & .01 & .01\\\cline{2-3}
%      & Meps15 & sex & .86&.02&.02&.01&-.16&.92 & .06 & .05 &\cellcolor{gray!10} .05 & \cellcolor{gray!45}.1 \\\cline{2-3}
%      & Meps16 & sex & .86&.03&.02&.02 &\cellcolor{gray!55}.63&.63&.65&.66&\cellcolor{gray!55}.67&\cellcolor{gray!55}.69 \\\cline{2-3}
%      & Students & sex & .91 & .01 & .02 & \cellcolor{gray!10}.06 & NV & NV & NV &NV & NV & NV \\\cline{2-3}\hline
    
%     \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race &.81&.01&.01&.01 &.08&.85 & .11 & .07 &\cellcolor{gray!10} .08 & \cellcolor{gray!10}.08\\
%     & & Sex & .81&.0&.0&.01 &\cellcolor{gray!65}1.00&.85 & .06 & .01 & -.03 & -.08\\\cline{2-3}
%     & Credit & Sex & .71&.21&.14&\cellcolor{gray!10}.09 &\cellcolor{gray!35}.32&.76 & .04 & .01 & .03 &\cellcolor{gray!10} .05\\\cline{2-3}
%     SVM & Bank & Age & .89&.11&.05&.01 &.03&.9 & .04 & .02 & .0 & -.04\\\cline{2-3}
%     & \multirow{3}{*}{Compas} & Sex & .95&.0&.02&-.04 &-.08&.94 & .0 & .02 & .0 & .0 \\  
%     &  &  Race &  .96&.0&.01&-.02 &-.06&.95 & .0 & .01 & .0 & -.04 \\
%     & &  Age & .95&.0&.0&-.01 &-.03&.94 & .0 & .02 & .0 & -.01 \\\cline{2-13} 
%      & Default & sex & .8 & .01& .0 & .0 & .0 &.84 & .02 & .02 & .0 & -.05 \\\cline{2-3}
%      & Heart & sex & .84&.0&.01&\cellcolor{gray!10}.06&.02&.79 & .08 & .06 & .0 & .0\\\cline{2-3}
%      & Meps15 & sex & .87&.0&.01&.0 &\cellcolor{gray!45}.42&.91 & .05 & .03 & .04 & \cellcolor{gray!45}.13 \\\cline{2-3}
%      & Meps16 & sex & .85&.02&.0&.01 &\cellcolor{gray!65}.88&.91 & .06 & .04 &\cellcolor{gray!10} .06 & \cellcolor{gray!55}.21 \\\cline{2-3}
%      & Students & sex &.93&.05&.0&\cellcolor{gray!10}.09 &\cellcolor{gray!65}.96&.91 & .02 & .04 & -.04 & -.05\\\cline{2-3}\hline

%      \multirow{9}{*}{Avg-based} & \multirow{2}{*}{Census} & Race &.84&.03&.02&\cellcolor{gray!10}.07&.01&.88 & .01 & .01 & \cellcolor{gray!10}.06 & -.22\\
%     & & Sex &.84&.01&.05&-.04&.0&.88 & .02 & .01 & .01 & \cellcolor{gray!10}.05\\\cline{2-3}
%     & Credit & Sex & .74&.34&.18&\cellcolor{gray!10}.05 &NV & .81 & .03 & .05 & .04 & \cellcolor{gray!45}.12 \\\cline{2-3}
%     RF & Bank & Age & .91&.03&.01&.01 &.01&.94 & .02 & .02 & -.03 & -.12 \\\cline{2-3}
%     & \multirow{3}{*}{Compas} & Sex & .94&.03&.02&-.03 &-.03&.93 & .01 & .0 & -.02 & .03 \\  
%     &  &  Race &  .93&.02&.0&-.03 &.0&.93 & .01 & .0 & -.04 & -.28 \\
%     & &  Age & .93&.02&.01&-.02 &.0&.93 & .01 & .01 & .05 & -.03\\\cline{2-13} 
%      & Default & sex &.79&.05&.03&.01&.01&.86 & .01 & .01 & .01 & .0\\\cline{2-3}
%      & Heart & sex &  .81&.37&.07&.03 &.0&.89 & .01 & .02 & .01 & -.07 \\\cline{2-3}
%      & Meps15 & sex & .85&.09&.06&.04&-.05&.91 & .02 & .01 & .03 & -.26 \\\cline{2-3}
%      & Meps16 & sex & .86&.01&.0&.0 &.0&.91 & .01 & .01 & .03 & \cellcolor{gray!10}.07\\\cline{2-3}
%      & Students & sex & .91& .03 & .09 & -.01 & NV & .91 & .01 & .01 & -.03 & -.09 \\\cline{2-3}\hline
%     \end{tabular}
%  }
%  \vspace{-1.0 em}
% \end{table*}


==> Sections/RQ-4-Table-bef_mj.tex <==
\setlength{\tabcolsep}{18pt} % Default value: 6pt
\begin{table*}[tbp!]
    \caption{Tail-Aware Bias mitigation.
      Legend is similar to Table~\ref{tab:EVT-Bias-Mitigation}
    % \textbf{P}: Protected Attribute,
    % \textbf{Acc$'$}: Accuracy of mitigated model,
    % \textbf{AOD}: AOD of original model,
    % \textbf{AOD$'$}: AOD of mitigated model,
    % \textbf{CVaR}: CVaR of original model,
    % \textbf{CVaR$'$}: CVaR of mitigated model.
    % \textbf{ECD$'$}: ECD$^2$ of mitigated model, 
    % \textbf{RLD}$'_{n}$: RLD for the next $n$ queries for mitigated model.           
    }
    \label{tab:CVaR-Bias-Mitigation}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{ | c | l  l |  c  c  c  c|   c  c  c   c | }
      \hline
      \multicolumn{3}{|c|}{\textbf{Name}}  &  \multicolumn{4}{c|}{\textbf{Minimax-Fairness~\cite{10.1145/3461702.3462523}}} & \multicolumn{4}{c|}{\textbf{ECD-Fairness}}
      \\
    \multicolumn{1}{|c}{Algorithm}  & Dataset  & P & Acc loss  & $|AOD|$ & $ACD$  & $ECD$ & Acc loss  & $|AOD| $& $ACD$  & $ECD$
    \\ \hline
    \multirow{4}{*}{DNN} & \multirow{2}{*}{Census} & Race & -.04 & .01 & -.04 & -.27  &.0  & .02 & \cellcolor{gray!20}.06 & .02\\
                           &                         & Sex  & -.04  & .03 & -.02 & -.07 &-.01  & .09 & -.06 & -.05\\ \cline{2-3}
    &  Credit                                        & Sex  & .-.07  & .01 & -.02 & -.02 &-.04  & .0 & .01 & .01\\ \cline{2-3}
    Tail-based & Bank                                       & Age & -.11  & .0 & .02 & .03  &-.04 & .03 & .0 & -.01\\ \cline{2-3}

    & \multirow{1}{*}{Compas}                        & Race & -.01  & .02 & .0 & \cellcolor{gray!20}.08 &.01 & .02 & -.01 & -.02\\ \cline{2-3}
    % & \multirow{3}{*}{Compas}                        & Sex  & .0  & .03 & .04 & -.11  &.0  & .03 & -.02 & .01\\
    % &                                                & Race & -.01  & .02 & .0 & \cellcolor{gray!10}.08 &.01 & .02 & -.01 & -.02\\ 
    % &                                                &  Age & .0  & .01 & .02 & \cellcolor{gray!10}.15  &.0  & .01 & .03 & .02\\ \cline{2-3}
     & Default                                       & Sex & .0  & .01 & -.01 & -.07  &.01  & .0 & .03 & .02\\ \cline{2-3}
     & Heart                                       & Sex & -.04 & .05 & .01 & .01  &.02  & .04 & -.03 & -.04\\ \cline{2-3}
     & Meps15                                       & Sex  & .01  & .01 & -.01 & -.03  &.02  & .03 &\cellcolor{gray!5} .05 & .04\\ \cline{2-3}
     & Meps16                                       & Sex  & .0 & .01 & .01 & .02  &.0 & .03 & \cellcolor{gray!20}.08 & \cellcolor{gray!40}.1\\ \cline{2-3}
     & Studens                                       & Sex & .0  & .03 & -.02 & -.1  &-.01  & .06 & -.01 & -.03\\ \cline{2-3}\hline
    \multirow{4}{*}{LR} & \multirow{2}{*}{Census} & Race &.0  & .05 & \cellcolor{gray!60}.17 & \cellcolor{gray!80}.2 &-.03  & .01 & .04 & .03\\
    &                                               & Sex &  .0 & .1 & -.07 & -.08&-.03  & .01 & -.01 & -.01\\ \cline{2-3}
    &  Credit                                       & Sex & .0 & .12 & \cellcolor{gray!60}.12 & \cellcolor{gray!60}.12 &-.02  & .04 & .04 & .04\\ \cline{2-3}
    Tail-based & Bank                                       & Age  & -.01 & .06 & -.02 & -.02&-.01& .04 & .03 & .04\\ \cline{2-3}

    & \multirow{1}{*}{Compas}                       &  Race & .0 &  .02 & .0 & -.04&.0  & .02 & -.02 & -.04\\  \cline{2-3}

    % & \multirow{3}{*}{Compas}                       & Sex & .0 & .03 & .0 & -.02&.0  & .03 & -.01 & -.02\\  
    % &                                               & Race & .0 &  .02 & .0 & -.04&.0  & .02 & -.02 & -.04\\
    % &                                               &  Age & .01 &  .01 & .0 & .02&.0 & .01 & .03 & .02\\ \cline{2-3}
    & Default                                       & Sex & .0 &  .03 & .03 & .03&-.01  & .02 & .01 & .01\\ \cline{2-3}
     & Heart                                       & Sex & -.09 &  .0 & .0 & .0&-.03 &  .1 & -.02 & -.04\\ \cline{2-3}
     & Meps15                                       & Sex  & -.04  & .0 & .0 &\cellcolor{gray!5} .05&-.01  & .04 & .02 & .03\\ \cline{2-3}
     & Meps16                                       & Sex  & -.02  & .01 & .01 &\cellcolor{gray!20} .08&.0  & .01 & .02 & .03\\ \cline{2-3}
     & Studens                                       & Sex & .01  & .01 & \cellcolor{gray!20}.07 & \cellcolor{gray!60}.18&-.01 & .02 & .0 & .0\\ \cline{2-3}\hline
    


    
    \end{tabular}
 }
\end{table*}    

==> Sections/background.tex <==
\section{Background}
\label{sec:prelim}

\textbf{Fairness in Machine Learning.} \stsays{candidate to remove!}
We focus on binary classification tasks where a \textit{favorable} label gives a benefit to an individual such as a low risk of default for loan applications, low risk of re-offending for parole assessments, and high qualification score for job hiring. Each dataset consists of a number of \textit{attributes} (e.g., income, employment status, job experiences, prior arrests, sex, and race) and a set of \textit{instances} that assign values to attributes for each individual. 
In our fairness setting, we label every attribute with either \textit{protected} or \textit{non-protected} tag. 
According to legal and ethical requirements, ML models should not \textit{discriminate} on the basis of protected attributes.

There are several well-established measures of fairness in ML.
\emph{Group Fairness} requires the statistics of ML outcomes for different
protected groups remain similar (e.g., female vs. male)~\cite{hardt2016equality}.
Examples of group fairness metrics include equal opportunity difference (EOD) and average odd difference (AOD)~\cite{bellamy2019ai}. EOD measures the difference in the true positive rates between two groups whereas AOD measures the average of differences in the true positive rates and false positive rates between two groups. 

\emph{Individual Fairness} (e.g., Fairness through awareness~\cite{dwork2012fairness}) requires two \textit{individuals}, who deem to be similar (based on their non-protected attributes), are treated similarly (regardless of their protected attributes). 
However, defining the notion of similarity between individuals are difficult. 
Counterfactual fairness~\cite{kusner2017counterfactual} uses causal dependency diagram between variables and require that the ML outcome is causally independent of protected attributes. 
Causal discrimination~\cite{agarwal2018automated,udeshi2018automated,zhang2020white,9793943}
defines a simpler notion of individual fairness (in the absence of an
explicit causal dependency graph) that requires the ML outcome to remain similar between the record of an individual
and their counterfactual record (differing only in the value of the protected attribute).
\textsc{Themis}~\cite{10.1145/3106237.3106277} extends this notion to define the \textit{average
causal discrimination} (ACD) that is the average differences of ML outcomes for 
individual samples with the protected attribute $p$ to their counterfactuals with 
the protected attributes are set to $u$.


\vspace{0.25em}
\noindent \textbf{Extreme Value Theory (EVT).} 
Extreme value theory~\cite{coles2001introduction} is a statistical branch that deals
with the analysis of extreme events in a random process.
Given a set of independent and identically distributed random variables $\set{z_1,\ldots,z_n}$, the extreme
value theory is concerned with the min/max statistics of a random process, i.e., $M_n = \max(\set{z_1,\ldots,z_n})$
or $M_n = \min(\set{z_1,\ldots,z_n})$ as $n \to \infty$. 

Under some mild assumptions, it has been proved (e.g., see Leadbetter et al.~\cite{leadbetter2012extremes}) that $Pr[(M_n-b_n)/a_n < z] \to G(z)$ as $n \to \infty$ and $G$ belongs to a family of distributions called the \emph{generalized extreme value (GEV)} family. Each such distribution has the CDF of
\[
G(z) = \exp\left\{-\left[1 + \xi\left(\frac{z - \mu}{\sigma}\right) \right]^{-1/\xi}\right\},
\]
defined over $\{z: 1 + \xi(z - \mu)/\sigma > 0\}$. 
The model has three parameters: a location parameter $-\infty<\mu<+\infty$, a scale parameter
$\sigma > 0$, and a shape parameter $-\infty < \xi < +\infty$. Type I, known as Gumbel family, defines for a subset of GEV distribution when $\xi \to 0$. The tail behavior of type I, $z_{+}$, has infinite support, but the density of GEV decays exponentially (guarantees are feasible up to a bounded interactions). For type II, $\xi > 0$ and $z_{+}$ has infinite support, decaying polynomially (limited guarantees may be feasible). For a special case where $\xi \geq 1$, the mean of GEV is infinite, decaying logarithmically, so no statistical guarantee is feasible. Finally, for type III, $\xi < 0$ and $z_{+}$ has finite support. In this case, the statistical guarantees on the worst-case outcomes are feasible for a long horizon.

\vspace{0.25em}
\noindent \textit{Generalized Pareto Distribution.} 
There are two basic approaches to infer the parameters of GEV distributions: block maximum and threshold approach. The block maximum approach divides samples into blocks of same size and use the maximum of each block as the extreme value. Since such approach is more appropriate for seasonal data, in this paper, we use the threshold approach where extreme events that exceed some high threshold $u$, i.e., $\{x_i: x_i > u\}$, are extreme values. Labeling these exceedances by
$\{\delta_{(1)},\ldots,\delta_{(k)}\}$, we define threshold excesses by $\delta_j = x_j - u$ for $1 {\leq} j {\leq} k$. It follows that if $Pr[M_n < z] \to G(z)$, then for large enough $u$, the distribution function of ($T-u$), conditional on $T>u$, is approximately 
\[
H(t) = 1 - \left(1 + \frac{{\xi}t}{\hat{\sigma}} \right)^{-1/\xi}
\]
where $t>0$ and $\hat{\sigma} = \sigma + \xi(u - \mu)$~\cite{coles2001introduction}.
This distribution is known as \textit{generalized Pareto} distribution. The implication of shape parameter $\xi$ is the
same as $G(z)$, as a special case of GEV distribution.

\vspace{0.5em}
\noindent \textit{Threshold Selection.} 
A proper choice of threshold value $u$ is critical to analyze the
behavior of extreme value distributions. Low values of threshold $u$ might
include non-tail samples and lead to mixture distributions that violate
the asymptotic basis of the model. On the other hand, high values of
threshold $u$ might include only a few tail samples and lead to low
confidence in the model due to high variance. Therefore, it is critical
to be confident on the threshold value to provide any guarantees on the
worst-case fairness behaviors. In this work, we use coefficient of variation
(CV) and provide statistical guarantees in picking thresholds. 

\vspace{0.5em}
\noindent \textit{Return Levels.}
It is often convenient to model extreme value distributions
using return levels. The inverse of probability density function of GEV at
probability $p$, is the \textit{return level} $\delta_p$,  associated with the
\textit{return period} $1/p$. Therefore, the level $\delta_p$ is expected
to be exceeded on average once every $1/p$ periods of time.
A \textit{return level} plot consists of points
{$(m,\delta_m)$} where $m$ is the time period (e.g., the number of interactions with the ML model) and the level $\delta_m$ is expected to exceed during the $m$ period (e.g., expected extreme discrimination in the next $m$ interactions).


